Measurement of the CKM angle gamma from a combination of B->Dh analyses

A combination of three LHCb measurements of the CKM angle gamma is presented. The decays B->DK and B->Dpi are used, where D denotes an admixture of D0 and D0-bar mesons, decaying into K+K-, pi+pi-, K+-pi-+, K+-pi-+pi+-pi-+, KSpi+pi-, or KSK+K- final states. All measurements use a dataset corresponding to 1.0 fb-1 of integrated luminosity. Combining results from B->DK decays alone a best-fit value of gamma = 72.0 deg is found, and confidence intervals are set gamma in [56.4,86.7] deg at 68% CL, gamma in [42.6,99.6] deg at 95% CL. The best-fit value of gamma found from a combination of results from B->Dpi decays alone, is gamma = 18.9 deg, and the confidence intervals gamma in [7.4,99.2] deg or [167.9,176.4] deg at 68% CL, are set, without constraint at 95% CL. The combination of results from B->DK and B->Dpi decays gives a best-fit value of gamma = 72.6 deg and the confidence intervals gamma in [55.4,82.3] deg at 68% CL, gamma in [40.2,92.7] deg at 95% CL are set. All values are expressed modulo 180 deg, and are obtained taking into account the effect of D0-D0bar mixing.

==> detector.tex <==
\section{Detector}
\label{sec:detector}
The \lhcb detector~\cite{Alves:2008zz} is a single-arm forward
spectrometer covering the \mbox{pseudorapidity} range $2<\eta <5$,
designed for the study of particles containing \bquark or \cquark
quarks. The detector includes a high precision tracking system
consisting of a silicon-strip vertex detector surrounding the $pp$
interaction region, a large-area silicon-strip detector located
upstream of a dipole magnet with a bending power of about
$4{\rm\,Tm}$, and three stations of silicon-strip detectors and straw
drift tubes placed downstream. The combined tracking system has
momentum resolution $\Delta p/p$ that varies from 0.4\% at 5\gevc to
0.6\% at 100\gevc, and impact parameter resolution of 20\mum for
tracks with high transverse momentum. Charged hadrons are identified
using two ring-imaging Cherenkov detectors. Photon, electron and
hadron candidates are identified by a calorimeter system consisting of
scintillating-pad and preshower detectors, an electromagnetic
calorimeter and a hadronic calorimeter. Muons are identified by a
system composed of alternating layers of iron and multiwire
proportional chambers. The trigger~\cite{Aaij:2012me} consists of a
hardware stage, based on information from the calorimeter and muon
systems, followed by a software stage which applies a full event
reconstruction.


